DocAsRef: An Empirical Study on Repurposing Reference-Based Summary Quality Metrics Reference-Freely

Automated summary quality assessment falls into two categories: reference-based and reference-free. Reference-based metrics, historically deemed more accurate due to the additional information provided by human-written references, are limited by their reliance on human input. In this paper, we hypothesize that the comparison methodologies used by some reference-based metrics to evaluate a system summary against its corresponding reference can be effectively adapted to assess it against its source document, thereby transforming these metrics into reference-free ones. Experimental results support this hypothesis. After being repurposed reference-freely, the zero-shot BERTScore using the pretrained DeBERTa-large-MNLI model of <0.5B parameters consistently outperforms its original reference-based version across various aspects on the SummEval and Newsroom datasets. It also excels in comparison to most existing reference-free metrics and closely competes with zero-shot summary evaluators based on GPT-3.5.

==> hebi_background.tex <==
\color{violet}

\textcolor{red}{(Hebi: Adding some formal equations so that readers/reviewers have a clear mind what we are talking about exactly. The details are generated by ChatGPT and needs verifying the correctness.)}

\subsection{Background: Reference-based Metrics}

There are four representative reference-based metrics, ROUGE~\cite{2004-Workshop-Lin-Rouge}, BERTScore~\cite{bert-score}, BLEURT~\cite{bleurt-sellam-etal-2020}, and MoverScore~\cite{zhao-etal-2019-moverscore}, formally defined as:

\begin{equation}
    \text{ROUGE} = \frac{{\text{{Overlapping n-grams}}}}{{\text{{Total n-grams in reference}}}}
\end{equation}

In the equation above, "Overlapping n-grams" refers to the count of n-grams (contiguous sequences of n words) that appear in both the generated summary and the reference summary. "Total n-grams in reference" represents the count of n-grams in the reference summary.

BERTScore is formally defined as:

\begin{equation}
    \text{BERTScore} = F1(\text{BERT}(sys), \text{BERT}(ref))
\end{equation}

In this equation, "sys" represents the tokenized version of the generated summary, "ref" represents the tokenized version of the reference summary, "BERT" represents the BERT model used to generate contextualized word embeddings, and "F1" represents the F1 score calculation between the embeddings of the generated and reference tokens.

\begin{equation}
\text{BLEURT} = \frac{1}{N} \sum_{i=1}^{N} \log P(y_i|x_i)
\end{equation}

In this equation, "BLEURT" represents the BLEURT score, "N" represents the total number of evaluation instances, $P(y_i|x_i)$ represents the probability assigned by the BLEURT model to the human score $y_i$ given the input pair $x_i$". BLEURT is a reference-based metric that uses a pre-trained model to estimate the similarity between generated summaries and their corresponding reference summaries.

\begin{equation}
\text{MoverScore} = \frac{1}{N} \sum_{i=1}^{N} \frac{\sum_{j=1}^{n} \max_{k=1}^{m} \text{sim}(r_{ij}, w_{ik})}{n}
\end{equation}

In this equation, $MoverScore$ represents the MoverScore, $N$ represents the total number of evaluation instances, $m$ represents the number of words in the generated summary, $n$ represents the number of words in the reference summary, $w_{ij}$ represents the j-th word in the generated summary, $r_{ik}$ represents the k-th word in the reference summary, and $similarity(w_{ij}, r_{ik})$ represents the similarity score between the words.

MoverScore is a reference-based metric that measures the amount of "movement" required to transform the generated summary into the reference summary. It computes the similarity between each word in the generated summary and the reference summary, and then takes the maximum similarity value for each generated word, which is divided by the total number of generated words (m) to obtain the average score.


\subsection{Background: Reference-free Metrics}

Requiring highly educated human labor, reference summaries are very costly to obtain. 
% Hence, the use of reference-based metrics is limited and very difficult in industrial applications. 
Therefore, many reference-free metrics have emerged recently
% such as SummaQA~\cite{scialom-etal-2019-answers}, BLANC~\cite{vasilyev-etal-2020-fill}, and SueNes~\cite{suenes}, 
~\cite{scialom-etal-2019-answers, vasilyev-etal-2020-fill, suenes},
which directly compute a score between a system summary and its source document.

\begin{equation}
\text{score} = \text{Similarity}\left(\text{systemSum}, \text{Doc}\right)
\end{equation}

In this equation, "Similarity" represents a function that measures the similarity between the generated summary and the context in which it is generated. The context can include the original document, additional information, or other contextual cues. Reference-free metrics aim to evaluate the quality of summaries without the need for explicit reference summaries.

\subsection{Repurposing Ref-based to Ref-free}

This section formally describe how we repurpose reference-based metrics to reference free.

Given the effectiveness of reference-based metrics in comparing a summary and a reference, we propose repurposing these metrics to directly compare a summary and the source document. This approach transforms a reference-based metric into a reference-free metric, enabling evaluation without relying on reference summaries. To identify reference-based metrics with potential for such repurposing, we benchmark four representative metrics, namely ROUGE~\cite{2004-Workshop-Lin-Rouge}, BERTScore~\cite{bert-score}, BLEURT~\cite{bleurt-sellam-etal-2020}, and MoverScore~\cite{zhao-etal-2019-moverscore}, on four representative datasets (\S~\ref{Exp:settings}). Instead of using references, we feed these metrics with the source documents as inputs (Appendix~\ref{sec:appendix:code}).

Let's denote the repurposed reference-free metric as $\text{RepurposedMetric}$, which measures the similarity between a summary and the source document. The equation to formally describe this approach can be represented as follows:

\begin{equation}
\text{Repurposed} = \text{Metric}(Sum, \text{Doc})
\end{equation}

In this equation, $\text{Metric}$ represents the chosen reference-based metric (e.g., ROUGE, BERTScore, BLEURT, MoverScore) applied to compare the summary with the source document. The inputs to the $\text{Metric}$ function are the generated summary and the source document itself, replacing the traditional reference summaries used in the reference-based evaluation. This repurposing enables the evaluation of summary quality without relying on explicit reference summaries.

Specifically, the repurposed ROUGE is formally,

\begin{equation}
    \text{ROUGE}' = \text{ROUGE}(Sum, Doc)
\end{equation}

the repurposed BERTScore is,

\begin{equation}
    \text{BERTScore}' = \text{BERTScore}(Sum, Doc)
\end{equation}

The repurposed BERTscore using the RoBERTa-large-MNLI langauge model (LM) \textcolor{red}{(Hebi: we should probably outline how exactly the different LMs come into play with the BERTScore, as many LMs are evaluated in the experiments.)}:

\begin{equation}
\text{BERTScore}' = \text{RoBERTa-L-MNLI}(Sum, Doc)
\end{equation}

The inputs to the "BERTScore" function are the generated summary (Summary), the source document (SourceDocument), and the RoBERTa-large-MNLI language model (\text{RoBERTa-large-MNLI}). The RoBERTa-large-MNLI model is used to compute the contextualized word embeddings and similarity scores between the summary and the source document.

This repurposing allows for the evaluation of summary quality without relying on explicit references, enabling the direct comparison between the summary and the source document using the specified language model.

\color{black}
